Planning and Control of Uncertain Cooperative Mobile Manipulator-Endowed Systems under Temporal-Logic Tasks

Control and planning of multi-agent systems is an active and increasingly studied topic of research, with many practical applications such as rescue missions, security, surveillance, and transportation. This thesis addresses the planning and control of multi-agent systems under temporal logic tasks. The considered systems concern complex, robotic, manipulator-endowed systems, which can coordinate in order to execute complicated tasks, including object manipulation/transportation. Motivated by real-life scenarios, we take into account high-order dynamics subject to model uncertainties and unknown disturbances. Our approach is based on the integration of tools from the areas of multi-agent systems, intelligent control theory, cooperative object manipulation, discrete abstraction design of multi-agent-object systems, and formal verification. The first part of the thesis is devoted to the design of continuous control protocols for cooperative object manipulation/transportation by multiple robotic agents, and the relation of rigid cooperative manipulation schemes to multi-agent formation. In the second part of the thesis, we develop control schemes for the continuous coordination of multi-agent complex systems with uncertain dynamics, focusing on multi-agent navigation with collision specifications in obstacle-cluttered environments. The third part of the thesis is focused on the planning and control of multi-agent and multi-agent-object systems subject to complex tasks expressed as temporal logic formulas. The fourth and final part of the thesis focuses on several extension schemes for single-agent setups, such as motion planning under timed temporal tasks and asymptotic reference tracking for unknown systems while respecting funnel constraints.

==> SetUps/KTHLicentiate.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Packages
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\usepackage{ifdraft}

\usepackage{lmodern}
\usepackage{textcomp}
\usepackage[utf8x]{inputenc}
\usepackage[english]{babel}
%\usepackage[swedish,english]{babel}
\usepackage{amsfonts}
\usepackage{amsmath}
\usepackage{amssymb}
\usepackage{amsthm}
%\usepackage{MnSymbol}% By persahl
\usepackage{multirow} % By persahl

\usepackage[final,dvips]{graphicx}
\usepackage{url}
\usepackage{tabulary}
\setlength{\tymin}{100pt}
% Special hack below to break the damn URL!
\def\UrlBreaks{\do\.\do\@\do\\\do\/\do\!\do\_\do\|\do\;\do\>\do\]%
 \do\)\do\,\do\?\do\'\do+\do\=\do\#\do\i\do\m\do\t\do\a\do\x}%

\usepackage[numbers,sort&compress]{natbib}
%\usepackage{cite}
\usepackage[config, font={small}, labelfont={bf}, margin={3mm}]{caption}
\usepackage{subcaption}
\usepackage{lettrine}
\usepackage[final]{microtype}
\usepackage{marvosym}
\usepackage[table]{xcolor}
\usepackage{hyphenat}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Show comments or not
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%5
\ifdraft{}{\commentsoff{comment}}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%5

%%%%%%%%%%%%%%%%%%%%%55
% Citation style and fixes
%%%%%%%%%%%%%%%%%%%%%%%%%%
%% For Per style uncomment the following four lines /Pablo

%\bibliographystyle{persahl_thesis}
%\bibpunct{(}{)}{;}{y}{,}{,}
%\newcommand{\citeasnoun}{\citet}
%\renewcommand{\cite}{\citep}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Theorem environments
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\newtheorem{theorem}{Theorem}
\numberwithin{theorem}{chapter}
\newtheorem{lemma}{Lemma}
\numberwithin{lemma}{chapter}
\newtheorem{conjecture}{Conjecture}
\newtheorem{corollary}{Corollary}
\theoremstyle{definition}
\newtheorem{proposition}{Proposition}
\newtheorem{definition}{Definition}
\numberwithin{definition}{chapter}
\newtheorem{remark}{Remark}
\numberwithin{remark}{chapter}
\newtheorem{assumption}{Assumption}
\numberwithin{assumption}{chapter}
\newtheorem{example}{Example}
\numberwithin{example}{chapter}
\newtheorem{problem}{Problem}
\numberwithin{problem}{chapter}
\newtheorem{property}{Property}
\numberwithin{property}{chapter}


%%%%%%%%%%%%%%%%%%%55
% Style fixes
%%%%%%%%%%%%%%%%%%%%%%%

%%% Chapterstyle
\makeatletter

% Fix TOC
\renewcommand{\@pnumwidth}{3em}
\renewcommand{\@tocrmarg}{4em}

\makechapterstyle{per}{
	\renewcommand{\printchaptername}{\raggedleft}
	\renewcommand{\printchapternum}{\chapnumfont \chaptername\ \thechapter}
	\renewcommand{\chapnumfont}{\normalfont\LARGE\sffamily}
	\renewcommand{\chaptitlefont}{\normalfont\Huge\sffamily}
	%\renewcommand{\chapnumfont}{\normalfont\LARGE}
	%\renewcommand{\chaptitlefont}{\normalfont\Huge}
	\renewcommand{\printchaptertitle}[1]{%
	\vspace{-9mm}
	\rule{\textwidth}{1pt}\\[.25mm]
	\chaptitlefont \raggedleft ##1 \\
	\vspace{-3.75mm} \rule{\textwidth}{1pt} \\\vspace{-4mm}}
	\renewcommand{\afterchaptertitle}{\vskip \afterchapskip}
} \makeatother
\chapterstyle{per}

\frenchspacing

\setlength{\parskip}{0pt}
%\setlength{\epigraphwidth}{9cm}
\setlength{\epigraphwidth}{10cm}
\setlength{\epigraphrule}{0pt}

\pagestyle{companion}
\makeevenhead{companion}%
{\normalfont\sffamily\thepage}{}{\normalfont\sffamily\leftmark {}}
\makeoddhead{companion}%
{\normalfont\sffamily\rightmark {}}{}{\normalfont\sffamily\thepage}
\setlength{\headwidth}{\textwidth}
\renewcommand{\labelitemii}{}

\renewcommand{\arraystretch}{1.2}
\renewcommand{\bf}{\bfseries}
\newcommand{\scr}{\scriptscriptstyle}
%\maxtocdepth{subsection} \settocdepth{subsection}
\maxsecnumdepth{subsection} \setsecnumdepth{subsection}

\widowpenalty=1000 \clubpenalty=1000
%\addtolength{\abovecaptionskip}{-2mm}
%\addtolength{\abovecaptionskip}{-1mm}
%\addtolength{\belowcaptionskip}{-2mm}
%\addtolength{\floatsep}{-2mm}
